Transforming and Projecting Images into Class-conditional Generative Networks

We present a method for projecting an input image into the space of a class-conditional generative neural network. We propose a method that optimizes for transformation to counteract the model biases in generative neural networks. Specifically, we demonstrate that one can solve for image translation, scale, and global color transformation, during the projection optimization to address the object-center bias and color bias of a Generative Adversarial Network. This projection process poses a difficult optimization problem, and purely gradient-based optimizations fail to find good solutions. We describe a hybrid optimization strategy that finds good projections by estimating transformations and class parameters. We show the effectiveness of our method on real images and further demonstrate how the corresponding projections lead to better editability of these images.

==> deprecated/basincma_ablation.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.6\linewidth]{./images/basincma_ablation.pdf}
    \vspace{-.1in}
    \caption{\small \textbf{How CMA and gradient updates affect performance:} We plot VGG L-PIPS score -- lower is better -- as a function of CMA updates (x-axis) and the number of ADAM updates (y-axis). The right balance of ADAM and CMA updates leads to the best result.}
    \label{fig:basincma_updates}
    \vspace{-.1in}
\end{figure}


==> deprecated/biggan_size.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=1.0\linewidth]{./images/comp_size.pdf}
    \vspace{-.28in}
    \caption{\small \textbf{Object size comparison} We use an off-the-shelf object detector to compute the distribution of object widths ({\bf left}) and heights ({\bf right}). Note that ImageNet (darker blue) has a long-tail, whereas BigGAN (lighter blue) generates objects closer to the distribution mode.}
    \label{fig:comp_size}
    \vspace{-.1in}
\end{figure}


==> deprecated/biggan_stats.tex <==

\begin{figure}[t!]
    \centering
    \includegraphics[width=1.0\linewidth]{./images/comp_center.pdf}
    \vspace{-.30in}
    \caption{\small \textbf{Object center comparison} We use off-the-shelf object detector to compute the histogram of object locations. Note that ImageNet ({\bf left}) is biased towards the center but exhibits a long-tail. BigGAN ({\bf right}) is further biased towards center.}
    \label{fig:comp_center}
    \vspace{-.1in}
\end{figure}



==> deprecated/class_error.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.5\linewidth]{./images/class_error.pdf}
    \caption{\small \textbf{Reconstruction error by class:} The average VGG-perceptual loss with standard error.
    %  for each superclass in PASCAL.
    The ImageNet images are sampled from the PASCAL super-class.}
    \label{fig:class_error}
\end{figure}


==> deprecated/class_search.tex <==
\setlength{\tabcolsep}{4pt}
\begin{table}[t]
\begin{center}
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{lcccc} 
    \toprule
    & \multicolumn{4}{c}{\textbf{Best of 9 seeds}} \\ \cmidrule(lr){2-5} 
    
    \multirow{2}{*}{\bf Class search}  & \multicolumn{2}{c}{\bf Per-pixel} & \multicolumn{2}{c}{\bf LPIPS} \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5} 
    & \textbf{L1} & \textbf{L2} & \textbf{Alex} & \textbf{VGG} \\ 
    \midrule
Random Gaussian            & 1.26 & 0.88 & 0.69 & 0.86 \\
Random Class               & 0.88 & 0.51 & 0.40 & 0.59 \\
Predicted                  & 0.83 & 0.47 & 0.33 & 0.51 \\ \cdashline{1-5}
Ground Truth               & 0.82 & 0.47 & 0.32 & 0.50 \\
\bottomrule
\end{tabular}
}
\caption{\small \textbf{Class search:} Given a fixed optimization method (ADAM + Transform), we compare different methods for initializing the class vector (lower is better). We provide few baselines: the projected class vector is randomly initialized from the normal distribution, a random class is given, and as an oracle we provide the ground truth image.}
\label{table:cls_pred}
\end{center}
\end{table}

==> deprecated/coco.tex <==
\setlength{\tabcolsep}{4pt}
\begin{table}[t]
\begin{center}
%72.7 & 35.0
\resizebox{0.7\linewidth}{!}{
\begin{tabular}{l cccc} 
    \toprule
    & \multicolumn{4}{c}{\textbf{Best of 9 seeds}} \\ \cmidrule(lr){2-5}  
    
    \multirow{2}{*}{\bf Method} & \multicolumn{2}{c}{\bf Per-pixel} & \multicolumn{2}{c}{\bf LPIPS} \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5} 
    & \textbf{L1} & \textbf{L2} & \textbf{Alex} & \textbf{VGG} \\ 
    \midrule
ADAM                    & 0.32 & 0.19 & 0.32 & 0.56 \\
ADAM + Transform        & 0.27 & 0.15 & 0.39 & 0.52 \\
BasinCMA                & 0.31 & 0.18 & \textbf{0.27} & 0.53 \\ 
BasinCMA + Transform    & \textbf{0.26} & \textbf{0.14} & 0.36 & \textbf{0.49} \\
\bottomrule
\end{tabular}
}
\caption{\small \textbf{Out-of-distribution:} We compare different methods on the COCO-dataset (lower is better). The class labels are predicted using ResNext-101 and the masks are predicted using MaskRCNN.}
\label{table:coco}
\end{center}
\end{table}
    


==> deprecated/failures.tex <==
\begin{figure*}[t!]
    \centering
    % \includegraphics[width=\linewidth]{./images/failures.pdf}
    \includegraphics[width=\linewidth]{./images/failures_v2.pdf}
    \vspace{-.25in}
    \caption{\small \textbf{Failure cases:} Typical failure cases of our method. Our method fails to invert images that are not well represented by BigGAN. }
    \label{fig:failures}
    \vspace{-.05in}
\end{figure*}


==> deprecated/oldtext.tex <==
\section{Background}
Although our method is not limited to GANs, we focus on solving the inversion problem of Generative Adversarial Networks (GANs), as it is the most popular method for image synthesis. We will first state the GAN formulation and the inversion problem before describing our proposed method.

\subsection{Generative Adversarial Networks (GANs)}
A generative adversarial network (GAN) is a family of generative models that consists of 2 networks: a generator G and a discriminator D. These networks are parameterized by deep neural networks. The goal of the generator is to model the data distribution $Y$ from a latent noise vector $z$: 

\begin{equation}
    G(z) = \hat{y}.
\end{equation}

This latent vector $z$ is sampled from a known distribution, such as the normal distribution $z \sim \mathcal{N}(0, I)$. The goal of the generator is to generate a sample $\hat{y}$ that is indistinguishable from $y \in Y$. This results in a min-max objective formulation, where the goal of the generator is to maximize the log-likelihood of fooling the discriminator with the generated samples, while the goal of the discriminator is to discriminate all fake samples from real samples:

\small
\begin{equation}\label{eq:gan}
    \min_G \max_D \mathbb{E}_{y \sim q_{data}}[\log D(y)] + \mathbb{E}_{z \sim p_{z}}[\log(1 - D(G(z))].
\end{equation}
\normalsize

Here $q_{data}$ is the real data distribution, and $p_z$ is the sample distribution. In this work, we focus on BigGAN~\cite{}, a state-of-the-art GAN model for class-conditional image generation on ImageNet~\cite{}.

\subsection{Image Inversion}
GANs, once trained, can learn a meaningful latent representation that can be used as a low-dimensional controller for high-level image manipulations. With recent works demonstrating the edit-ability of generated images~\cite{}, there has been an increased interest in finding the corresponding latent vectors for \textit{real images}. Of course, majority of these real images will not have a corresponding $z$ vector and will require us to find the best approximation. This task requires one to solve for the following optimization:

\begin{equation}\label{eq:inv}
    \min_{z} \mathcal{L}( G(z), y) \quad s.t \quad C(z) \leq \epsilon.
\end{equation}

Here the $\mathcal{L}$, is a distance function that measures how far the generated image is from the target image $y$, and $C$ is a set of constraints for the latent vector $z$ that needs to be satisfied. $C(z)$ is non-negative and $C(z) = 0$ if and only if all the constraints are satisfied. Here an example of a constraint that we use is that the latent vector must be close to the original sampling distribution, $|z| \leq 2$. We can soften up the constraints by controlling for $\epsilon$, but larger the $\epsilon$, the more likely the resulting optimization will result in solutions that fall off the sampling distributions -- solutions that may recover the target image but is not meaningful (e.g., cannot be edited). Note that the exact solution to the above equation where $\mathcal{L} = 0$ and $C(z)=0$ can only be guaranteed for images generated by $G$.

One would expect that optimizing a low-dimensional $z$ vector would be straight-forward, but the complexity of the generative model $G$ makes the optimization non-trivial. Hence, the choice of loss functions, variable constraints, and optimization techniques are all important components to finding a good latent approximation. In our work, we explore the facets that are required to successfully invert arbitrary image into the latent manifold. 


\subsection{Transformation and Invertibility Loss}
Generative adversarial networks are not spatially invariant; that is, a GAN may not be able to invert a generated image that has been shifted by a few pixels. The spatial dependency of the generator raises the possibility that even if the object in the image had a close approximate solution in the generative model, we might not be able to invert the image at all if it is not in the right location. 
For example, in \fig{} we measure the sensitivity of the optimization as the generated images are shifted horizontally. 

%that by simply placing the image into the mean distribution of images that the model generates, we can find a better solution. The types of transformations the generative model is sensitive to are not limited to spatial transformations, but also color transformations of the image such as saturation, hue, and so on. 

%TALK ABOUT BIGGAN
Another insight we can get is by observing what the generative model is capable of generating. It is a well-known fact that GANs are susceptible to mode collapse and are not able to precisely model the training data distribution. We can quantify this by running an off-the-shelf object detector to compute the average shape and location of the generated image and compare it to the statistics in the training images. In ~\fig{}, we observe that BigGAN does not model the long tail distribution of images and has a shape and location it favors. Spatially transforming the real image accordingly, we can achieve better inversion.

This motivates the idea of optimizing for image transformation such that the inversion optimization becomes more tractable. We can reformulate the optimization objective as:

\begin{equation}
\min_{z, \Phi} \mathcal{L}( G(z), \Phi(y)) \quad s.t \quad C(z) \leq \epsilon.
\end{equation}

Instead of optimizing for $z$ alone, we additionally optimize for image transformation $\Phi$, where the transformation can be an arbitrary invertible function. For example, one can consider the simplest case of an affine transformation where we assume there is no sheering:

\begin{equation}
\Phi = \begin{bmatrix}
s_x & 0 & t_x \\
0 & s_y & t_y \\
\end{bmatrix}
\end{equation}

Here $s_x, s_y$ scales the image and $t_x, t_y$ translates the image in $x, y$ coordinates respectively. To solve for the optimal $\Phi$, one can search over all possible locations at every scale, but this can be computationally intractable. One potential approach is to not optimize for the transformation at all and transform the image into the generative model's typical output shape. Conversely, one can consider optimizing the transformation $\Phi$ through optimization using gradient descent or BasinCMA.


\subsection{Class recognition}
\jacob{this doesnt seem to improve any better than predicted class vector, we should remove it. we do optimize it with gradient descent on the continuous vector.}
\aaron{I’m thinking this should go before optimization algorithms, but it depends. Have we tried directly optimizing c with gradient descent, or does the GAN not work with continuous c inputs? Doesn’t it have a continuous embedding that we could optimize in?}

For conditional GANs, additional class information is provided to the generative model:
\begin{equation}
\by = G(\bz, \bc),
\end{equation}
where $c$ is the discrete one-hot encoded class vector. This class vector is embedded into a continuous vector using the generator's class encoder $G_{E}$. 
Since discrete value optimization is difficult to optimize, we instead directly optimize over the embedded class vector~\cite{}. 

\jacob{this needs to be re-written}
Because the projected class vectors do not come from a well-defined distribution, optimizing over randomly initialized class vectors will not work well. In the case where the class information is not available, we found that using a pre-trained classification model to work almost as well. For both the ground-truth class vector and the predicted class vector, we optimize the project embedding instead of the onehot class encoding.

\comm{
    Although state-of-the-art classification models can achieve high accuracy, wrong initial guesses can be difficult to overcome. 
    To reduce the margin of error given by the classification model, we propose the idea of optimizing over the linear combination of the top classification queries. Given a pre-trained classification model $F_{cls}$, we denote the output of the $k$-th highest prediction of an input image $x$ as $F_{cls}(x, k)=c_{k}, p_{k}$, where $c_k$ is the predicted class and $p_k$ is the associated probability. We then use the generative model to embed these discrete class vectors into continuous vectors $E(c_k) = \bar{c}_k$. Given the number of top-$K$ classes we want to search over, we construct a class vector as a linear combination with the top $K$ predictions:
    
    \begin{equation}
    \hat{c} = \sum_{k}^{K} \bar{c}_k \hat{p}_k = \sum_{k}^{K}E(c_k) \frac{e^{p_k}}{\sum_{j \in K} e^{p_j}}
    \end{equation}
    
    Here $\hat{p_k}$ is the softmax normalized output probabilities of $p_k$. Instead of optimizing for $c_k$ or $\bar{c}_k$, we optimize for the scalar probability coefficients $\hat{p}_k$. This reduces the class search space into a smaller subspace.
}




One approach would be to use a large number of random initial seeds (in the order of 100s) as proposed in~\cite{}, but this would require a tremendous amount of computation time to find a good solution, even then we show that in the appendix that this it is not guaranteed. % cma outperforms model trained with 100 seeds.
Recent works~\cite{bau, jeffdonaaronuebijection} have proposed to use a trained encoder network to mitigate these shortcomings, but they are complicated to train and do not always provide a robust solution. %Trained encoders, however, do provide a good initial guess of the latent vector, and we explore using it jointly with our method. 
Unlike previously explored methods, we wish to find an optimization technique that is: 1) resilient to local minima, 2) model-agnostic, 3) robust without an encoder. \aaron{and fast?} % BasinCMA is not fast, CMA is fast.
To this end, we revisit the use of gradient-free optimization method \textit{Covariance Matrix Adaptation Evolution Strategies} (CMA)~\cite{}, which demonstrated great success in solving non-convex problems. 

We consider the following optimizers:

\renewcommand\labelitemi{$\vcenter{\hbox{\tiny$\bullet$}}$}
\begin{itemize}[leftmargin=*]
    \item \textbf{ADAM} \cite{tbd} and \textbf{L-BFGS} \cite{tbd}, two state-of-the-art gradient based optimizers.
    \item \textbf{Encoder,} A model trained to predict $\bz$ from an input image~\cite{}.
    \item \textbf{CMA,} The CMA algorithm is a gradient-free numerical optimizer that is extremely good at avoiding local minima. For details of the algorithm, see \cite{tbd}. CMA requires an initial parameter estimate, which we provide as a zero vector, and an covariance matrix, for which we provide an identity matrix. We also experimented with BasinCMA 
    \item \textbf{BasinCMA} \cite{tbd}, but did not find that it improved results
    \item \textbf{Combinations.} \aaron{explain ADAM + CMA, ADAM + Encoder, etc}
\end{itemize}

\aaron{old text below that I think can be removed}

\xpar{CMA}
CMA starts with an initial guess of a distribution $\mathcal{N}(\mu_0, \mathcal{C}_0)$, where we set $\mu_0 = 0$ and set $\mathcal{C} = I$ (the identity matrix). The CMA distribution is a guess of the latent vector that minimizes the objective function. $N$ candidates are sampled from this distribution $z_{i} \sim \mathcal{N}(\mu_k, \mathcal{C}_k)$, where $k$ is the $k$-th iteration of the algorithm. The algorithm evaluates and ranks individual candidates $f(z_i)$, where  $f(\cdot)$ is the optimization objective function in \eqn{inv_w_per}. From these rankings, we update the mean and the covariance matrix. For simplicity, we will write this update rule as:

\begin{equation}\label{eq:inv}
    \mu_{k+1}, \mathcal{C}_{k+1} \leftarrow Update(\mu_k, \mathcal{C}_k, \{f(z_i)\}_{i=0}^{N}).
\end{equation}

The full update rule can be referred from ~\cite{} or can be seen in the appendix~\ref{}. Once trained, we sample latent vectors from the CMA distribution and optimize it using gradient descent.
We demonstrate the effectiveness of using CMA in \fig{} and further observed substantial improvements in robustness and downstream editing. 

\xpar{Hybrid Optimization (BasinCMA\cite{})} We build upon the success of using CMA and explore the use of gradient optimization jointly with CMA. This hybrid optimization has been used in graphics for synthesizing locomotion~\cite{}. In BasinCMA, instead of directly updating the CMA distribution on the sampled candidates $\{z_i\}_{i=0}^{N}$, we update the CMA using the expected loss after optimizing the latent vectors with gradient descent. This equates to taking $t_b$ gradient steps on the sample $\{z_i\}_{i=0}^{N}$. For an arbitrary optimizer $\Omega$, we can make a simple change to the update rule:
\begin{equation}\label{eq:inv}
    \mu_{k+1}, \mathcal{C}_{k+1} \leftarrow Update(\mu_k, \mathcal{C}_k, \{\Omega^{t_b} (z_i, f)\}_{i=0}^{N}).
\end{equation}
Here $\Omega$ optimizes the latent vector $z_i$ using the loss function $f$ for $t_b$ steps. We will refer to this method as BasinCMA from here forth. In ~\fig{}, we observed that the hybrid-optimization is more robust than CMA.
%We discuss the speed versus quality trade-off off in the appendix~\ref{}.

\comm{
    To observe which methods can best find the transformation for the downstream optimization, in \fig{}, we manually apply a translation to the generated images to see which search methods can best recover the applied translation. Since the images were generated from the generator, we know there exists an exact solution at a unique location. 
}


\subsection{Fine-tuning}


%\input{figures/translation}

==> deprecated/translation.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{./images/translation.pdf}
    \vspace{-.25in}
    \caption{\small \textbf{Recovering Translation:} Generated images are translated horizontally, we compare how well each methods can recover the inverse transformation.}
    \label{fig:translation}
\end{figure}


==> figures/class_vector_study.tex <==
\begin{figure}[t]
\begin{minipage}[b]{.49\textwidth}
\centering
\includegraphics[width=1.0\linewidth]{./images/class_vector_tsne.pdf}
\vspace{-0.1in}
\caption{\small \textbf{Class vector t-SNE:} The t-SNE embedding of the optimized class vector after optimization. The color represents the class and the circles with black border are the original classes.}
\label{fig:cv_tsne}
\end{minipage}
\hfill
\begin{minipage}[b]{.49\textwidth}
\centering
\includegraphics[width=1.0\linewidth]{./images/optimize_class_vector.pdf}
\vspace{-0.1in}
\caption{\small \textbf{Class deviations:} Optimizing the class-vector directly leads to large deviation from the ground-truth vector. We instead optimize for the linear combination coefficients of top predictions.}
\label{fig:cv_opt_err}
\end{minipage}
\vspace{-0.2in}
\end{figure}

